Fair-Net: A Network Architecture For Reducing Performance Disparity Between Identifiable Sub-Populations

In real world datasets, particular groups are under-represented, much rarer than others, and machine learning classifiers will often preform worse on under-represented populations. This problem is aggravated across many domains where datasets are class imbalanced, with a minority class far rarer than the majority class. Naive approaches to handle under-representation and class imbalance include training sub-population specific classifiers that handle class imbalance or training a global classifier that overlooks sub-population disparities and aims to achieve high overall accuracy by handling class imbalance. In this study, we find that these approaches are vulnerable in class imbalanced datasets with minority sub-populations. We introduced Fair-Net, a branched multitask neural network architecture that improves both classification accuracy and probability calibration across identifiable sub-populations in class imbalanced datasets. Fair-Nets is a straightforward extension to the output layer and error function of a network, so can be incorporated in far more complex architectures. Empirical studies with three real world benchmark datasets demonstrate that Fair-Net improves classification and calibration performance, substantially reducing performance disparity between gender and racial sub-populations.

==> backup_tables.tex <==

\begin{table*}[!htb]
\centering
\caption{Variation of predictive performance across sub-populations for adult census dataset. }
\begin{tabular}{cccc}
\toprule
                                               & F-measure ($\mu \pm \sigma$)  & ROC AUC ($\mu \pm \sigma$)   & ECE ($\mu \pm \sigma$) \\
									           \cmidrule(r){2-4}

Fair-Net Branched                              & \textbf{0.69 $\pm$ 0.016}    & \textit{0.917} $\pm$ \textbf{0.024}  & \textit{0.016 $\pm$ 0.01}      \\
Fair-Net Branched [histogram loss]             & \textit{0.689 $\pm$ 0.018}    & \textit{0.917} $\pm$ 0.027                    & \textbf{0.015 $\pm$ 0.008}       \\
Fair-Net Un-Branched                           & 0.681 $\pm$ 0.025             & 0.916 $\pm$ 0.026                    & 0.021 $\pm$ 0.013     \\
Fair-Net Un-Branched [histogram loss]          & 0.686 $\pm$ 0.019             & \textbf{0.918} $\pm$ 0.027           & 0.019 $\pm$ \textbf{0.008}     \\\cmidrule(r){2-4}
Cal-Net                                        & 0.68  $\pm$ 0.024             & \textit{0.917} $\pm$ 0.026                    & 0.017 $\pm$ \textbf{0.008}     \\
Baseline NN [balanced xent]                    & 0.679 $\pm$ 0.029             & 0.91 $\pm$ 0.026                     & 0.058 $\pm$ 0.023     \\
Sub-population Specific                        & 0.631 $\pm$ 0.06              & 0.894 $\pm$ \textit{0.025}           & 0.102 $\pm$ 0.019      \\\bottomrule
\end{tabular}	
\label{tab:variations}
\end{table*}
